EBGAN-MDN: An Energy-Based Adversarial Framework for Multi-Modal Behavior Cloning

Multi-modal behavior cloning faces significant challenges due to mode averaging and mode collapse, where traditional models fail to capture diverse input-output mappings. This problem is critical in applications like robotics, where modeling multiple valid actions ensures both performance and safety. We propose EBGAN-MDN, a framework that integrates energy-based models, Mixture Density Networks (MDNs), and adversarial training. By leveraging a modified InfoNCE loss and an energy-enforced MDN loss, EBGAN-MDN effectively addresses these challenges. Experiments on synthetic and robotic benchmarks demonstrate superior performance, establishing EBGAN-MDN as a effective and efficient solution for multi-modal learning tasks.

==> DL_project/EBGAN_app.tex <==
\section{The Failure of EBGAN} \label{Failure_GAN_app}
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\linewidth]{Diagran_EBGAN.png}
    \caption{Enter Caption}
    \label{fig:enter-label}
\end{figure}


\begin{figure}[h!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.5\linewidth]{DL_project/asset/LatentSpaceCollabse.png}}
\caption{XXX No title in image - we need to cut that}
\label{fig:Latent_space_collabse}
\end{center}
\vskip -0.2in
\end{figure}


==> DL_project/report.tex <==
\section{Proposal}
\textcolor{magenta}{Julia: use as ref for completeness w.r.t. the proposal when writing. Exclude for final submission.}
\subsection{Introduction}
Label ambiguity arises in machine learning when a single input corresponds to multiple valid outputs. This issue is particularly problematic for methods like Behavior Cloning (BC) in robotics, which trains agents to mimic demonstrations using supervised learning. By assuming unimodality \cite{NEURIPS2022_90d17e88}, traditional BC approaches average over conflicting samples, often producing unsafe or nonsensical predictions. For example, minimizing mean squared error loss in such scenarios leads to erratic approximations, as shown in Fig.~\ref{fig:example_hyperbola}. 

Various approaches attempt to address multimodal conflicts in BC. Filtering strategies \cite{florence2022implicit} remove conflicting samples but require explicit mode identification, which is impractical for complex tasks. Energy-based models (EBMs), such as Implicit Behavior Cloning (IBC) \cite{zamora2022learning}, learn low-energy manifolds to capture multimodal distributions but are computationally expensive due to iterative optimization during inference. 
Beyond BC, imitation learning methods like Generative Adversarial Imitation Learning (GAIL) \cite{NIPS2016_cc7e2b87} use adversarial training to match agent and expert state-action distributions but fail in multimodal settings by interpolating between modes, as seen in Fig.~\ref{fig:example_hyperbola} and \cite{ke2020imitationlearningfdivergenceminimization}.

We propose Energy-Based Generative Adversarial Networks for Behavior Cloning (EBGAN-BC) to address these challenges. 


% \textcolor{red}{Our approach has shown effectiveness in early tests (code available at \url{github.com/zipping-suger/MultiModLearn}) and} offers a scalable solution to multimodal conflicts in BC.

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\textwidth]{asset/Two-Link_IK.png}
%     \caption{Learning results on a two-link robotic arm inverse kinematics problem. Each target position can be reached by two different joint configurations (elbow-up and elbow-down modes). 
%     The heat map shows the error between target points and forward kinematics of predicted configurations. The MSE-MLP learns an average between the two valid configurations, producing invalid solutions. GAN generates more precise individual poses.}
%     \label{fig:example_two_link_ik}
% \end{figure*}

% \section{Background}
% \subsection{Behavior Cloning}
% Behavior cloning (BC) is a supervised learning approach where a policy is learned directly from demonstration data. 
% The goal is to mimic the behavior of an expert by learning a mapping from states to action \cite{ravichandar2020recent}. 
% This is typically achieved by minimizing the MSE between the predicted actions and the demonstrated actions.

% \subsection{Energy-based Models}
% Energy-based models (EBMs) assign scalar energy values to input-output pairs, with lower energy indicating plausibility. They capture multimodal distributions effectively but face challenges in scalability due to high computational costs and reliance on task-specific gradients, especially in high-dimensional spaces.

% \subsection{Generative Adversarial Networks}
% Generative Adversarial Networks (GANs) \cite{NIPS2014_5ca3e9b1} consist of a generator, which synthesizes data, and a discriminator, which distinguishes between real and generated samples. 
% While GANs naturally model multimodal distributions and allow efficient sampling, they are prone to mode collapse, where generated outputs fail to capture the diversity of the underlying data.

\subsection{Methods}
EBGAN-BC replaces the traditional GAN discriminator with an energy model $E$, which assigns low energy to expert actions and high energy to generated actions. The generator $G$ learns to mimic expert demonstrations by minimizing the energy of its outputs. Unlike prior work on energy-based GANs \cite{zhao2017energybased}, which uses a reconstruction loss for image generation, EBGAN-BC employs an InfoNCE-based loss \cite{oord2018representation}, a novel approach tailored to address multimodal conflicts in behavior cloning.

By combining the strengths of EBMs and generative adversarial networks (GANs) \cite{NIPS2014_5ca3e9b1}, EBGAN-BC aims to efficiently model multimodal distributions. Its adversarial training mechanism enables diverse outputs without explicit mode identification, while the energy-based formulation accurately captures the data’s structure. Unlike traditional EBMs, EBGAN-BC avoids iterative optimization during inference, ensuring scalability.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.85\columnwidth]{DL_project/asset/Hyperbola_3.png}
    \caption{Learning results on a two-valued hyperbola: The ground truth (black points) shows two valid y-values per x-input. The MSE-based MLP averages modes (red), EBMs capture both but generate suboptimal samples, GANs collapse to one mode, while EBGAN-BC accurately learns both modes with a clear energy landscape.}
    \label{fig:example_hyperbola}
\end{figure}
\vspace{-10pt}
% Given expert actions \(x\) and generated and counter sampled actions \(G(z)\), along with the energy function \(E\), the losses are defined as:
% \begin{equation}
% \mathcal{L}_E = \text{InfoNCE}(E(x), E(G(z)))
% \end{equation}
% \begin{equation}
% \mathcal{L}_G(z) = E(G(z))
% \end{equation}
% Validation on a two-valued hyperbola function (Fig.~\ref{fig:example_hyperbola}) shows EBGAN-BC effectively captures distinct modes and generates high-quality samples without mode collapse.

\subsection{Experiments}
Our experiments evaluate EBGAN-BC's ability to handle multimodal distributions and its scalability, efficiency, and performance compared to baseline methods. We aim to determine if EBGAN-BC can learn from multimodal distributions without mode collapse, how it performs relative to baseline methods, and its inference speed.

We compare EBGAN-BC to three baselines: vanilla BC, which uses MSE loss for supervised learning and MLPs; Implicit Behavior Cloning (IBC) \cite{florence2022implicit}; and standard GAIL methods \cite{NIPS2016_cc7e2b87}. 

\subsection{Tasks and Datasets}
We evaluate EBGAN-BC on a variety of problems: toy problems including a multi-value hyperbola and a two-link inverse kinematics problem, robot manipulation tasks (simulated pushing, planar sweeping, and bi-manual sweeping), and the D4RL benchmark \cite{fu2020d4rl}, which includes real-world robotic datasets. The synthetic tasks, excluding D4RL, allow controlled experiments on multimodality and complexity.



==> DL_project/summary.tex <==
\section{Summary}


Add paper:
\url{https://arxiv.org/pdf/2206.11251}
